Using Petri Nets as an Integrated Constraint Mechanism for Reinforcement Learning Tasks

The lack of trust in algorithms is usually an issue when using Reinforcement Learning (RL) agents for control in real-world domains such as production plants, autonomous vehicles, or traffic-related infrastructure, partly due to the lack of verifiability of the model itself. In such scenarios, Petri nets (PNs) are often available for flowcharts or process steps, as they are versatile and standardized. In order to facilitate integration of RL models and as a step towards increasing AI trustworthiness, we propose an approach that uses PNs with three main advantages over typical RL approaches: Firstly, the agent can now easily be modeled with a combined state including both external environmental observations and agent-specific state information from a given PN. Secondly, we can enforce constraints for state-dependent actions through the inherent PN model. And lastly, we can increase trustworthiness by verifying PN properties through techniques such as model checking. We test our approach on a typical four-way intersection traffic light control setting and present our results, beating cycle-based baselines.

==> graphics/environmentSetup.tex <==
\begin{tikzpicture}

	\node[thick,draw,rounded corners=2,anchor=base,minimum height=30pt, align=center] (agent) at (0,0) {agent \\};
	\node[thick,draw,rounded corners=2,anchor=base] (env) at (3,0) {env};
	\node[thick,draw,rounded corners=2,anchor=base,minimum height=30pt,align=center] (constraints) at (3,0) {constraints \\};
	
	\draw[->,transform canvas={yshift=2pt}] (agent) -- node[above] {actions} (constraints);
	\draw[->,transform canvas={yshift=-2pt}] (constraints) -- node[below] {$\mathcal{X}$} (agent);
\end{tikzpicture}

==> graphics/results/evaluation-results-table.tex <==
\newcommand{\hl}[1]{\textbf{#1}}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[]
% \centering
% \begin{tabular}{|l|l|ccc|ccc|cc|}
% \hline
% \multirow{2}{*}{\textbf{Model Name}} & \multirow{2}{*}{\textbf{Model Parameters}} & \multicolumn{3}{c|}{\textbf{timesteps}}    & \multicolumn{3}{c|}{\textbf{constraints broken}} & \multicolumn{2}{c|}{\textbf{waiting time}} \\
%                                      &                                            & \textbf{min} & \textbf{avg} & \textbf{max} & \textbf{min}   & \textbf{avg}   & \textbf{max}   & \textbf{avg}         & \textbf{max}        \\ \hline
% \multirow{8}{*}{DQN}                 & s=1.5 c=0.0 w=1.0 mw=1.5 t=0.0             & 41           & 547          & 1000         & 1.100\%        & \hl{8.026\%}   & \hl{17.600\%}  & 7.736                & \hl{36.160}              \\
%                                      & s=1.0 c=0.0 w=1.0 mw=1.5 t=0.0             & 12           & 572          & 1000         & \hl{0.400\%}   & 18.914\%       & 36.500\%       & 8.723                & 39.820              \\
%                                      & s=1.5 c=0.0 w=1.0 mw=0.0 t=0.0             & 18           & 652          & 1000         & 1.600\%        & 19.074\%       & 33.800\%       & 8.638                & 41.825              \\
%                                      & s=2.0 c=0.0 w=1.0 mw=0.0 t=0.0             & 11           & 707          & 1000         & \hl{0.900\%}        & \hl{15.129\%}  & \hl{24.700\%}  & 8.697                & 40.645              \\
%                                      & s=1.0 c=0.0 w=1.0 mw=0.0 t=0.0             & \hl{65}     & 745          & 1000         & 1.800\%        & 29.961\%       & 46.100\%       & 7.893                & 42.560              \\
%                                      & s=2.0 c=0.0 w=1.0 mw=1.5 t=0.0             & 36           & 774          & 1000         & \hl{0.900\%}        & 26.896\%       & 41.200\%       & 8.780                & 43.670              \\
%                                      & s=0.0 c=0.0 w=1.0 mw=0.0 t=0.0             & 54           & \hl{881}     & 1000         & 2.800\%        & 38.411\%       & 46.800\%       & \hl{7.484}                & 39.660              \\
%                                      & s=0.0 c=0.0 w=1.0 mw=1.5 t=0.0             & \hl{95}      & \hl{899}     & 1000         & 3.900\%        & 35.717\%       & 42.500\%       & \hl{7.313}                & \hl{37.725}              \\ \hline
% \multirow{3}{*}{CDQN}                & c=1.0 w=1.0 mw=1.5 t=0.0                   & 11           & \hl{100}          & \hl{200}          & \hl{3.000\%}        & \hl{10.638\%}       & 19.000\%       & 10.349               & 46.935              \\
%                                      & c=0.0 w=1.0 mw=1.5 t=0.0                   & \hl{47}           & 93           & 157          & 4.459\%        & 10.815\%       & \hl{17.834\%}       & 10.513               & 46.830              \\
%                                      & c=0.0 w=1.0 mw=0.0 t=0.0                   & 26           & 83           & 159          & 5.660\%        & 13.868\%       & 22.642\%       & 10.254               & 43.235              \\ \hline
% \multirow{2}{*}{Baseline}            & v2 (4, 5, 6, 7, 1, 8, 2, 0, 8, 3)          & \hl{66}           & \hl{150}           & \hl{326}          & 0.000\%        & 0.000\%        & 0.000\%        & 11.705           & 50.470         \\
%                                      & v1 (4, 5, 6, 7, 1, 2, 0, 3)                & 43           & 61           & 85           & 0.000\%        & 0.000\%        & 0.000\%        & \hl{9.570}           & \hl{30.160}         \\ \hline
% \end{tabular}
% \label{tab:evaluation-results}
% \caption{Best 8 trained agents run (each 200 times)}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|ccc|ccc|cc|}
\hline
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Model Parameters}} & \multicolumn{3}{c|}{\textbf{Timesteps}}    & \multicolumn{3}{c|}{\textbf{Constraints violated}} & \multicolumn{2}{c|}{\textbf{AJWT}} \\
                                     &                                            & \textbf{min} & \textbf{avg} & \textbf{max} & \textbf{min}   & \textbf{avg}   & \textbf{max}   & \textbf{avg}         & \textbf{max}        \\ \hline
\multirow{8}{*}{DQN}                 & $w_0$=1.5 $w_1$=0.0 $w_2$=1.0 $w_3$=1.5 $w_4$=0.0            & 129          & 869          & 1000         & \hl{3.500\%}   & \hl{14.097\%}  & \hl{25.500\%}  & 8.389                & 43.085              \\
                                     & $w_0$=1.0 $w_1$=0.0 $w_2$=1.0 $w_3$=1.5 $w_4$=0.0             & 138          & 848          & 1000         & 6.900\%        & 28.711\%       & 37.900\%       & 9.048                & 45.695              \\
                                     & $w_0$=1.5 $w_1$=0.0 $w_2$=1.0 $w_3$=0.0 $w_4$=0.0             & 141          & 963          & 1000         & 7.800\%        & 27.964\%       & 35.700\%       & 8.765                & 44.475              \\
                                     & $w_0$=2.0 $w_1$=0.0 $w_2$=1.0 $w_3$=0.0 $w_4$=0.0             & 120          & 942          & 1000         & 4.800\%        & \hl{19.525\%}  & \hl{25.500\%}  & 8.931                & 44.275              \\
                                     & $w_0$=1.0 $w_1$=0.0 $w_2$=1.0 $w_3$=0.0 $w_4$=0.0             & 68           & 946          & 1000         & \hl{3.900\%}   & 38.285\%       & 46.300\%       & 7.992                & 44.720              \\
                                     & $w_0$=2.0 $w_1$=0.0 $w_2$=1.0 $w_3$=1.5 $w_4$=0.0             & 115          & 960          & 1000         & 6.900\%        & 33.577\%       & 39.900\%       & 8.859                & 45.600              \\
                                     & $w_0$=0.0 $w_1$=0.0 $w_2$=1.0 $w_3$=0.0 $w_4$=0.0             & \hl{370}     & \hl{984}     & 1000         & 17.300\%       & 42.927\%       & 47.400\%       & \hl{7.551}           & \hl{41.655}         \\
                                     & $w_0$=0.0 $w_1$=0.0 $w_2$=1.0 $w_3$=1.5 $w_4$=0.0             & \hl{207}     & \hl{987}     & 1000         & 10.500\%       & 39.274\%       & 43.100\%       & \hl{7.387}           & \hl{39.695}         \\ \hline
\multirow{3}{*}{PN-CDQN}                &       $w_1$=1.0 $w_2$=1.0 $w_3$=1.5 $w_4$=0.0                   & 85           & 290     & 1000     & 0.000\%        & 0.000\%        & 0.000\%        & \hl{19.441}               & \hl{95.075}              \\
                                     &          $w_1$=0.0 $w_2$=1.0 $w_3$=1.5 $w_4$=0.0                   & 97      & 314           & 1000          & 0.000\%        & 0.000\%        & 0.000\%        & 25.434               & 100.405              \\
                                     &          $w_1$=0.0 $w_2$=1.0 $w_3$=0.0 $w_4$=0.0                   & \hl{115}           & \hl{520}           & 1000          & 0.000\%        & 0.000\%        & 0.000\%        &     27.079               & 103.765              \\ \hline
\multirow{2}{*}{Baseline}            & v2        & \hl{66}      & \hl{150}     & \hl{326}     & 0.000\%        & 0.000\%        & 0.000\%        & 11.705               & 50.470              \\
                                     & v1             & 43           & 61           & 85           & 0.000\%        & 0.000\%        & 0.000\%        & \hl{9.570}           & \hl{30.160}         \\ \hline
\end{tabular}
}
\caption{8 trained DQN agents with different constraint factors compared to the new developed PN-CDQN as well as the baseline version. All agent simulations are run 200 times and numbers shown are the minimum (min), average (avg) and maximum (values) reached. For timesteps, higher values equate to a better performance, whereas lower values are best for the percentage of constraint violations and the \textit{AJWT}.}
\label{tab:evaluation-results}
\end{table*}
